Deep Neural Network based Distance Estimation for Geometry Calibration in Acoustic Sensor Networks

We present an approach to deep neural network based (DNN-based) distance estimation in reverberant rooms for supporting geometry calibration tasks in wireless acoustic sensor networks. Signal diffuseness information from acoustic signals is aggregated via the coherent-to-diffuse power ratio to obtain a distance-related feature, which is mapped to a source-to-microphone distance estimate by means of a DNN. This information is then combined with direction-of-arrival estimates from compact microphone arrays to infer the geometry of the sensor network. Unlike many other approaches to geometry calibration, the proposed scheme does only require that the sampling clocks of the sensor nodes are roughly synchronized. In simulations we show that the proposed DNN-based distance estimator generalizes to unseen acoustic environments and that precise estimates of the sensor node positions are obtained.

==> simulations.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TeX root = Gburrek2020.tex
% !TeX program = pdflatex

\section{Simulation Results}
\label{sec:Sim}

\subsection{Simulation Framework}
For evaluation of our approach as well as for training of the \glspl{DNN}, simulated data is used.
In order to generate this data, the image method~\cite{image_source} is used to simulate \glspl{RIR}, whereby we utilize the \gls{RIR} generator from \cite{habets_rir}.
These are utilized to reverberate white Gaussian noise and speech, which stems from the TIMIT database~\cite{timit}, respectively.
Moreover, \gls{AWGN} is added to the reverberated signal in some experiments, in order to simulate sensor noise.
When generating the training data, the \gls{SNR} is chosen uniformly out of the interval [\SI{5}{\decibel}, \SI{30}{\decibel}]

The training and evaluation dataset for the distance estimator consists of single source-node pairs.
We consider the 2 dimensional case for all scenarios, which are examined in this paper.
Thus, all nodes and sources are placed in the plane $z=\SI{1.5}{\metre}$.
The nodes are placed uniformly in the room in all datasets, that correspond to the distance estimator.
Due to the fact, that the accuracy of distance estimates degrades, when the source or the node are located in the vicinity of walls, a minimal distance of \SI{0.5}{\metre} to the next wall is ensured for all nodes and sources.   

We consider separate datasets for the training of the distance estimator and the R-vector extractor.
This is motivated by the mismatch in the training data of both models, when real data would be used to train the distance estimator.
In both datasets rooms with a hight of \SI{3}{\metre} are considered.
The base area of the rooms is uniformly chosen out of the interval [\SI{6}{\metre}, \SI{7}{\metre}] x [\SI{5}{\metre}, \SI{6}{\metre}] for the distance estimator and out of the interval [\SI{5}{\metre}, \SI{8}{\metre}] x [\SI{4}{\metre}, \SI{7}{\metre}] for the R-vector extractor.
Besides, the reverberation time $T_{60}$ is randomly drawn out of [\SI{0.2}{\second}, \SI{0.5}{\second}] for distance estimation and out of [\SI{0.1}{\second}, \SI{0.6}{\second}] for R-vector training, respectively.
We placed the sources uniformly in the area around the nodes in the distance estimator dataset, whereby the distance to the nodes is randomly chosen from [\SI{0.03}{\metre}, \SI{3}{\metre}].
Additionally, \gls{OoR} examples are added to the dataset.
In the R-vector dataset all sources are uniformly distributed in the room.
Both dataset, that are used for training, contain 10000 source-node pairs, whereby additional 1000 \gls{OoR} are optionally added.

\todo{Adjustments needed: Geometry calibration scenario (One node is placed uniformly in each of the garnished areas. All areas have a distance of \SI{0.5}{\metre} to the walls. The areas are separated by a space of \SI{1}{\metre})}
\todo{Number plus length of observations}
In order to evaluate our approach to geometry calibration, we consider a scenario with four node, which are distributed as shown in Fig. \ref{fig:calib_Setup}.
The sources, that correspond to the observations, are uniformly distributed in the room.
Thereby, a minimal distance of \SI{0.5}{\metre} to the next wall is guaranteed.
It is to mention that this observations can be interpreted as points, where a speaker, walking along a trajectory, is standing still.

\subsection{Model Configuration}
All \glspl{DNN} are trained using Adam~\cite{Adam} with a mini-batch size of 32 and a learning rate of $3\cdot10^{-4}$.
The \gls{STFT}, which is needed to estimate $\widehat{\text{CDR}}(l, k)$, utilizes a Blackman window with a length of \SI{25}{\milli\second} and \SI{10}{\milli\second} shift.
Additionally, we estimate the \glspl{PSD} for \gls{CDR} estimation recursively with $\lambda=0.95$, as it is for example described in \cite{brendel_probabilistic_2019}.
Furthermore, diffuseness is calculated for the frequencies between \SI{125}{\hertz} and \SI{3.5}{\kilo\hertz}, which corresponds to the area, where speech is active. 	
\subsection{Distance Estimation}
In this subsection we investigate our distance estimator.
Therefore, we utilize the \gls{MAE} as metric
\begin{align}
e_{AE} = \frac{1}{N}\sum_{n=1}^{N}|\hat{r}_n - r_n|,
\end{align}
whereby $r_n$ denotes the ground truth distance and $\hat{r}_n$ the distance estimate.
The used evaluation set contains 10000 source-node constellations, which results in $N=30000$ source-microphone-pair constellations.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/gp_comparison}
	\caption{Placeholder: Comparison of \gls{DNN} and \gls{GP} (Cumulative error rate)}
	\label{fig:comparison}
\end{figure}
\todo{mention Andreas's comment (see mail)}
Fig. \ref{fig:comparison} shows the comparison \gls{GP}-based and \gls{DNN}-based distance estimation. 
...

\begin{table}[th]
	\caption{Performance of the distance estimator for different types of signals and different architectures (Input signals have a length of \SI{3}{\second}. Sensor noise is neglected.)}
	\label{tab:dist_est_architecture}
	\centering
	\begin{tabular}{c c c c c}
		\toprule
		& &  &  \multicolumn{2}{c}{\textbf{MAE} / m} \\		
		\textbf{Architecture} & \textbf{Diffuseness} & \textbf{R-vector} &\textbf{Noise} &\textbf{Speech}\\
		\midrule
		\gls{MLP} &  & \checkmark & 0.176 & 0.151\\
		\gls{MLP} & \checkmark &  & 0.119 & 0.148\\
		\gls{MLP} & \checkmark & \checkmark & 0.064 & 0.070\\
		\gls{CRNN} & \checkmark & & 0.087 & 0.055 \\
		\gls{CRNN}  & \checkmark & \checkmark & 0.062 & 0.052\\
		\bottomrule
	\end{tabular}
\end{table}
Table \ref{tab:dist_est_architecture} provides results for distance estimation using different input signals and \gls{DNN} architectures.
It becomes obvious that the best results can be achieved, when a \gls{CRNN} is used and therefore time information can be utilized.
This holds especially for speech as input signal.
Additionally, R-vectors can be helpful to reduce the error in all cases.
Nevertheless, R-vectors have a vanishing effect, when a \gls{CRNN} is used and speech is the input signal.
This means that the diffuseness contains enough information about the environment.
Moreover, better results can be archived, when speech is used instead of white Gaussian noise.
Thus, it can be stated, that the sparsity of the spectrogram of speech is beneficial for gathering information about the environment from the diffuseness.

\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[th]
	\caption{\todo{influence of snr plus oor-detection for best speech model}}
	\label{tab:dist_est}
	\centering
	\begin{tabular}{c  c c  c c}
		\toprule
		\textbf{SNR/\decibel} & \textbf{Fusion} &\textbf{MAE}/m &\textbf{F}$_\mathbf{1}$-\textbf{score (\gls{OoR} Detection)}\\
		\midrule
		$\infty$ &  & 0.045 & 88.17\%\\
		$\infty$ &\checkmark  & 0.028 & 89.75\%\\
		30 &\checkmark  & x.xx & xx.xx\%\\
		20 &\checkmark  & x.xx & xx.xx\%\\
		10 &\checkmark  & x.xx & xx.xx\%\\
		5 &\checkmark  & x.xx & xx.xx\%\\
		\bottomrule
	\end{tabular}
\end{table}
\endgroup

\subsection{Geometry Calibration}
\begin{itemize}
	\item \gls{PE} as metric:
\end{itemize}
\begin{align}
e = |\hat{\mathbf{n}}-\mathbf{n}|
\end{align}

\begin{table}[th]
	\caption{Dependency of \gls{MPE}/\metre on distances used for scaling and reverberation time}
	\label{tab:calib}
	\centering
	\begin{tabular}{| c | c | c | c | c |}
		\hline
		\diagbox[]{Distances}{$T_{60}/\text{ms}$} & 200 & 300 & 400 & 500\\
		\hline
		Ground truth distances & x.xx & x.xx & x.xx & x.xx \\
		\hline
		Distance estimates & x.xx & x.xx & x.xx & x.xx  \\
		\hline
	\end{tabular}
\end{table}
